Efficient Unlearning through Maximizing Relearning Convergence Delay

Machine unlearning poses challenges in removing mislabeled, contaminated, or problematic data from a pretrained model. Current unlearning approaches and evaluation metrics are solely focused on model predictions, which limits insight into the model's true underlying data characteristics. To address this issue, we introduce a new metric called relearning convergence delay, which captures both changes in weight space and prediction space, providing a more comprehensive assessment of the model's understanding of the forgotten dataset. This metric can be used to assess the risk of forgotten data being recovered from the unlearned model. Based on this, we propose the Influence Eliminating Unlearning framework, which removes the influence of the forgetting set by degrading its performance and incorporates weight decay and injecting noise into the model's weights, while maintaining accuracy on the retaining set. Extensive experiments show that our method outperforms existing metrics and our proposed relearning convergence delay metric, approaching ideal unlearning performance. We provide theoretical guarantees, including exponential convergence and upper bounds, as well as empirical evidence of strong retention and resistance to relearning in both classification and generative unlearning tasks.

==> figs-step-size/cifar10/res/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 006.510) (0.00001, 007.780) (0.000001, 007.780) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 000.310) (0.00001, 001.520) (0.000001, 001.520) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 008.420) (0.00001, 009.060) (0.000001, 009.060) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 001.495) (0.00001, 002.209) (0.000001, 002.400) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 010.650) (0.00001, 012.210) (0.000001, 012.210) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.000) (0.00001, 005.110) (0.000001, 005.110) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 007.410) (0.00001, 007.150) (0.000001, 007.150) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 007.870) (0.00001, 007.090) (0.000001, 007.090) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 007.640) (0.00001, 009.180) (0.000001, 009.840) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 001.330) (0.00001, 001.630) (0.000001, 001.730) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 007.200) (0.00001, 008.630) (0.000001, 009.430) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 001.680) (0.00001, 002.356) (0.000001, 002.622) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 003.120) (0.00001, 004.400) (0.000001, 004.840) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 003.700) (0.00001, 004.060) (0.000001, 004.660) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 010.820) (0.00001, 009.650) (0.000001, 009.480) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 011.120) (0.00001, 008.800) (0.000001, 008.630) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 093.200) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 040.070) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 081.670) (0.00001, 100.940) (0.000001, 101.000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 067.667) (0.00001, 068.900) (0.000001, 078.290) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 012.390) (0.00001, 067.290) (0.000001, 099.710) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 101.000) (0.00001, 101.000) (0.000001, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 037.320) (0.00001, 059.030) (0.000001, 101.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 044.120) (0.00001, 098.090) (0.000001, 101.000) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 100.920) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 062.880) (0.00001, 094.730) (0.000001, 101.000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 078.740) (0.00001, 096.850) (0.000001, 101.000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 084.669) (0.00001, 097.758) (0.000001, 101.000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 012.580) (0.00001, 056.600) (0.000001, 096.650) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 100.690) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 040.060) (0.00001, 090.350) (0.000001, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 043.060) (0.00001, 096.690) (0.000001, 101.000) };
    \end{axis}
\end{tikzpicture}



==> figs-step-size/cifar10/vit/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 015.870) (0.00001, 017.040) (0.000001, 017.600) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 005.680) (0.00001, 006.570) (0.000001, 006.980) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 011.440) (0.00001, 015.470) (0.000001, 017.770) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.645) (0.00001, 007.684) (0.000001, 008.236) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 019.390) (0.00001, 021.590) (0.000001, 024.270) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.000) (0.00001, 006.960) (0.000001, 007.430) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 013.940) (0.00001, 015.190) (0.000001, 016.340) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 013.720) (0.00001, 015.010) (0.000001, 015.890) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 019.600) (0.00001, 021.040) (0.000001, 021.650) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 005.740) (0.00001, 006.590) (0.000001, 007.110) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 011.640) (0.00001, 015.990) (0.000001, 019.670) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 006.789) (0.00001, 007.810) (0.000001, 008.237) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 034.140) (0.00001, 036.870) (0.000001, 038.780) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 008.280) (0.00001, 009.200) (0.000001, 010.010) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 014.300) (0.00001, 016.310) (0.000001, 017.820) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 014.300) (0.00001, 016.340) (0.000001, 017.810) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 037.280) (0.00001, 065.770) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 005.570) (0.00001, 019.080) (0.000001, 082.690) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 013.830) (0.00001, 065.630) (0.000001, 100.770) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.456) (0.00001, 019.742) (0.000001, 047.823) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 033.120) (0.00001, 069.770) (0.000001, 099.720) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 005.260) (0.00001, 015.300) (0.000001, 064.020) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 011.800) (0.00001, 041.110) (0.000001, 101.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 015.770) (0.00001, 049.260) (0.000001, 093.810) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 053.050) (0.00001, 069.920) (0.000001, 084.200) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.710) (0.00001, 017.310) (0.000001, 064.600) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 018.290) (0.00001, 071.060) (0.000001, 099.580) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 007.903) (0.00001, 024.791) (0.000001, 070.134) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 049.330) (0.00001, 080.630) (0.000001, 098.850) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.410) (0.00001, 014.900) (0.000001, 055.010) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 027.930) (0.00001, 065.700) (0.000001, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 024.480) (0.00001, 056.810) (0.000001, 086.130) };
    \end{axis}
\end{tikzpicture}



==> figs-step-size/cifar100/res/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 026.100) (0.00001, 031.100) (0.000001, 032.780) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 017.950) (0.00001, 016.330) (0.000001, 016.620) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 027.340) (0.00001, 030.240) (0.000001, 031.460) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 007.208) (0.00001, 009.882) (0.000001, 010.647) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 039.660) (0.00001, 041.890) (0.000001, 042.990) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 024.900) (0.00001, 022.540) (0.000001, 022.900) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 034.840) (0.00001, 032.020) (0.000001, 032.300) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 033.250) (0.00001, 031.740) (0.000001, 031.720) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 026.540) (0.00001, 030.190) (0.000001, 031.800) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 019.430) (0.00001, 016.320) (0.000001, 016.490) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 031.400) (0.00001, 035.390) (0.000001, 037.320) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 007.537) (0.00001, 010.428) (0.000001, 011.613) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 044.760) (0.00001, 048.230) (0.000001, 050.330) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 019.660) (0.00001, 018.010) (0.000001, 018.640) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 033.470) (0.00001, 028.380) (0.000001, 027.960) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 031.470) (0.00001, 028.310) (0.000001, 029.080) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 101.000) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 041.632) (0.00001, 098.239) (0.000001, 100.990) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 099.910) (0.00001, 100.999) (0.000001, 101.000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 045.276) (0.00001, 056.155) (0.000001, 085.608) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 039.935) (0.00001, 095.642) (0.000001, 099.254) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 100.553) (0.00001, 100.940) (0.000001, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 064.752) (0.00001, 084.548) (0.000001, 101.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 064.272) (0.00001, 091.937) (0.000001, 101.000) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 101.000) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 042.257) (0.00001, 094.702) (0.000001, 100.933) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 099.097) (0.00001, 100.764) (0.000001, 100.921) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 100.131) (0.00001, 101.000) (0.000001, 101.000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 092.792) (0.00001, 099.366) (0.000001, 099.714) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 097.662) (0.00001, 100.853) (0.000001, 101.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 078.522) (0.00001, 084.965) (0.000001, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 076.637) (0.00001, 086.302) (0.000001, 101.000) };
    \end{axis}
\end{tikzpicture}



==> figs-step-size/cifar100/vit/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 039.810) (0.00001, 042.470) (0.000001, 043.870) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 004.060) (0.00001, 006.060) (0.000001, 007.110) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 032.650) (0.00001, 040.810) (0.000001, 045.310) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 009.259) (0.00001, 012.673) (0.000001, 013.854) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 044.620) (0.00001, 048.890) (0.000001, 051.420) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 011.470) (0.00001, 014.500) (0.000001, 015.730) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 028.900) (0.00001, 038.030) (0.000001, 042.220) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 029.030) (0.00001, 037.910) (0.000001, 041.940) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 044.920) (0.00001, 048.700) (0.000001, 049.760) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 003.980) (0.00001, 005.970) (0.000001, 006.790) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 030.820) (0.00001, 039.370) (0.000001, 044.300) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 008.373) (0.00001, 011.868) (0.000001, 013.231) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 042.010) (0.00001, 050.770) (0.000001, 054.250) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 010.950) (0.00001, 015.350) (0.000001, 017.120) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 031.050) (0.00001, 039.800) (0.000001, 043.760) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 031.050) (0.00001, 040.000) (0.000001, 043.970) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 089.060) (0.00001, 100.910) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 010.800) (0.00001, 045.130) (0.000001, 098.810) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 057.530) (0.00001, 100.780) (0.000001, 101.000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 004.034) (0.00001, 016.232) (0.000001, 043.138) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 045.890) (0.00001, 094.670) (0.000001, 100.420) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 027.770) (0.00001, 067.960) (0.000001, 100.980) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 018.660) (0.00001, 056.130) (0.000001, 099.740) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 034.150) (0.00001, 072.560) (0.000001, 101.000) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 093.322) (0.00001, 100.997) (0.000001, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 006.818) (0.00001, 030.007) (0.000001, 081.142) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 062.880) (0.00001, 100.764) (0.000001, 100.995) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 004.177) (0.00001, 020.728) (0.000001, 060.417) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 072.638) (0.00001, 099.560) (0.000001, 100.897) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 023.553) (0.00001, 058.098) (0.000001, 096.785) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 049.756) (0.00001, 089.123) (0.000001, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 041.542) (0.00001, 084.382) (0.000001, 101.000) };
    \end{axis}
\end{tikzpicture}



==> figs-step-size/fig.tex <==
\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 0000000) (0.00001, 0000000) (0.000001, 0000000) };
    \end{axis}
\end{tikzpicture}


==> figs-step-size/tiny/res/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=\LARGE step-size,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.3,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 049.500) (0.00001, 052.160) (0.000001, 053.260) };
          \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 042.770) (0.00001, 039.420) (0.000001, 039.510) };
          \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 044.350) (0.00001, 047.530) (0.000001, 048.980) };
          % \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 032.181) (0.00001, 034.672) (0.000001, 035.872) };
          % \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 045.980) (0.00001, 048.080) (0.000001, 049.600) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 053.920) (0.00001, 046.110) (0.000001, 045.740) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 050.510) (0.00001, 048.760) (0.000001, 049.410) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 050.090) (0.00001, 048.190) (0.000001, 048.560) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=\LARGE step-size,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 055.990) (0.00001, 055.710) (0.000001, 057.360) };
          % \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 046.000) (0.00001, 041.130) (0.000001, 040.860) };
          % \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 044.580) (0.00001, 046.420) (0.000001, 047.650) };
          \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 032.424) (0.00001, 035.194) (0.000001, 036.576) };
          \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 049.900) (0.00001, 051.990) (0.000001, 054.490) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 057.220) (0.00001, 048.460) (0.000001, 047.720) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 054.640) (0.00001, 051.990) (0.000001, 052.150) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 054.940) (0.00001, 052.020) (0.000001, 051.990) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=\LARGE step-size,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.3cm,draw=none,font=\small, at={(-0.3,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 088.967) (0.00001, 100.297) (0.000001, 101.000) };
          % \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 049.901) (0.00001, 068.715) (0.000001, 093.491) };
          % \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 077.152) (0.00001, 099.939) (0.000001, 100.948) };
          % \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 069.100) (0.00001, 070.862) (0.000001, 077.991) };
          % \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 078.649) (0.00001, 099.147) (0.000001, 100.639) };
          \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 075.339) (0.00001, 095.754) (0.000001, 100.630) };
          \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 063.013) (0.00001, 082.367) (0.000001, 096.853) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 070.877) (0.00001, 086.781) (0.000001, 099.547) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=\LARGE step-size,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 092.246) (0.00001, 100.162) (0.000001, 101.000) };
          % \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 051.451) (0.00001, 066.925) (0.000001, 088.003) };
          % \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 088.094) (0.00001, 100.378) (0.000001, 100.964) };
          % \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 072.607) (0.00001, 074.028) (0.000001, 082.796) };
          % \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 071.749) (0.00001, 098.399) (0.000001, 100.481) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 061.524) (0.00001, 078.052) (0.000001, 093.646) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 074.276) (0.00001, 092.976) (0.000001, 098.681) };
          \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 067.574) (0.00001, 086.982) (0.000001, 097.890) };
    \end{axis}
\end{tikzpicture}



==> figs-step-size/tiny/vit/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0.0001, 062.710) (0.00001, 064.070) (0.000001, 064.540) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 058.210) (0.00001, 059.860) (0.000001, 060.580) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0.0001, 058.190) (0.00001, 059.570) (0.000001, 059.230) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 055.460) (0.00001, 056.794) (0.000001, 057.460) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 065.820) (0.00001, 067.840) (0.000001, 068.980) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 058.360) (0.00001, 059.990) (0.000001, 060.650) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 057.910) (0.00001, 059.860) (0.000001, 060.680) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 057.920) (0.00001, 059.780) (0.000001, 060.520) };
    \end{axis}
\end{tikzpicture}


\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 065.280) (0.00001, 067.290) (0.000001, 068.490) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 058.630) (0.00001, 060.450) (0.000001, 061.550) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 058.350) (0.00001, 059.760) (0.000001, 059.720) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0.0001, 056.863) (0.00001, 058.419) (0.000001, 059.222) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0.0001, 066.400) (0.00001, 070.180) (0.000001, 071.940) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 061.550) (0.00001, 064.150) (0.000001, 066.290) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 060.810) (0.00001, 064.090) (0.000001, 066.040) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 060.960) (0.00001, 064.230) (0.000001, 066.230) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 079.402) (0.00001, 084.332) (0.000001, 089.139) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 052.635) (0.00001, 064.593) (0.000001, 085.754) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 060.394) (0.00001, 085.206) (0.000001, 100.992) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 053.087) (0.00001, 063.731) (0.000001, 087.826) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 068.232) (0.00001, 094.145) (0.000001, 100.806) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 058.650) (0.00001, 074.434) (0.000001, 093.589) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 066.574) (0.00001, 086.889) (0.000001, 097.388) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 061.757) (0.00001, 078.623) (0.000001, 094.666) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[xmode=log,
                grid, xlabel=step-size,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0.0001, 087.784) (0.00001, 093.971) (0.000001, 097.569) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 051.872) (0.00001, 062.286) (0.000001, 080.032) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 064.515) (0.00001, 088.449) (0.000001, 100.914) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 052.327) (0.00001, 059.989) (0.000001, 073.583) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 076.719) (0.00001, 097.182) (0.000001, 100.795) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 049.997) (0.00001, 060.145) (0.000001, 079.230) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0.0001, 052.536) (0.00001, 063.480) (0.000001, 080.707) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0.0001, 053.512) (0.00001, 064.598) (0.000001, 082.376) };
    \end{axis}
\end{tikzpicture}



==> figs/cifar10/res/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (000.000, 006.510) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (000.020, 000.310) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (000.013, 008.420) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.026, 001.495) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.041, 010.650) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.021, 006.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.007, 007.410) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.008, 007.870) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 007.640) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.029, 001.330) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.011, 007.200) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (000.041, 001.680) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (000.021, 003.120) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.033, 003.700) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.015, 010.820) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.007, 011.120) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 093.200) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 040.070) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 081.670) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.004, 067.667) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.010, 012.390) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.002, 101.000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.006, 037.320) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 044.120) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.004, 062.880) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.008, 078.740) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 084.669) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.014, 012.580) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.000, 100.690) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.002, 040.060) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (000.001, 043.060) };
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 100.920) };
    \end{axis}
\end{tikzpicture}


==> figs/cifar10/vit/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (000.000, 015.870) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (000.043, 005.680) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (000.014, 011.440) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.037, 006.645) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.083, 019.390) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.040, 006.000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.018, 013.940) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.017, 013.720) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 019.600) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.065, 005.740) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.013, 011.640) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (000.065, 006.789) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (000.168, 034.140) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.054, 008.280) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.012, 014.300) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.016, 014.300) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 037.280) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.019, 005.570) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.016, 013.830) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.012, 006.456) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.067, 033.120) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.019, 005.260) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.007, 011.800) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.004, 015.770) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 053.050) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.012, 006.710) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 018.290) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.010, 007.903) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.033, 049.330) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.008, 006.410) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.006, 027.930) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (000.007, 024.480) };
    \end{axis}
\end{tikzpicture}


==> figs/cifar100/res/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)}, xticklabel style={font=\tiny},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (000.000, 026.100) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (000.045, 017.950) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (000.004, 027.340) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.076, 007.208) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.126, 039.660) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.026, 024.900) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.010, 034.840) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.012, 033.250) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 026.540) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.042, 019.430) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.055, 031.400) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (000.076, 007.537) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (000.202, 044.760) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.042, 019.660) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.028, 033.470) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.026, 031.470) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.004, 041.632) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 099.910) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.008, 045.276) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.034, 039.935) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.001, 100.553) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.003, 064.752) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 064.272) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 101.000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.006, 042.257) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.004, 099.097) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.009, 100.131) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.094, 092.792) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.002, 097.662) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.003, 078.522) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (000.003, 076.637) };
    \end{axis}
\end{tikzpicture}


==> figs/cifar100/vit/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (000.000, 039.810) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (000.091, 004.060) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (000.024, 032.650) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.080, 009.259) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.152, 044.620) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.071, 011.470) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.024, 028.900) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.027, 029.030) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)}, xticklabel style={font=\tiny},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 044.920) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.129, 003.980) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.037, 030.820) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (000.117, 008.373) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (000.145, 042.010) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.098, 010.950) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.016, 031.050) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.013, 031.050) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 089.060) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.001, 010.800) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.004, 057.530) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.010, 004.034) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.063, 045.890) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.001, 027.770) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.005, 018.660) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.009, 034.150) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 093.322) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.021, 006.818) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.005, 062.880) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.035, 004.177) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.091, 072.638) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.001, 023.553) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.006, 049.756) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (000.006, 041.542) };
    \end{axis}
\end{tikzpicture}


==> figs/fig.tex <==
\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (0000000, 0000000) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (0000000, 0000000) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (0000000, 0000000) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (0000000, 0000000) };
    \end{axis}
\end{tikzpicture}

==> figs/tiny/res/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=\LARGE Avg. Gap,
                 ylabel={\LARGE $\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\Huge, at={(-0.35,-0.25)}, xticklabel style={font=\tiny},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (000.000, 049.500) };
          \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (000.050, 042.770) };
          \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (000.059, 044.350) };
          % \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.054, 032.181) };
          % \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.115, 045.980) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.024, 053.920) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.024, 050.510) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.027, 050.090) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=\LARGE Avg. Gap,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.1,-0.25)}, xticklabel style={font=\tiny},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 055.990) };
          % \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.066, 046.000) };
          % \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.068, 044.580) };
          \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (000.076, 032.424) };
          \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (000.118, 049.900) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.031, 057.220) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.026, 054.640) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.028, 054.940) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=\LARGE Avg. Gap,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.3cm,draw=none,font=\small, at={(-0.3,-0.25)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 088.967) };
          % \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.012, 049.901) };
          % \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.025, 077.152) };
          % \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.037, 069.100) };
          % \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.095, 078.649) };
          \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.013, 075.339) };
          \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.012, 063.013) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.014, 070.877) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=\LARGE Avg. Gap,
                 ylabel=\LARGE {$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.25)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\huge Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 092.246) };
          % \addlegendentry{\huge FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.013, 051.451) };
          % \addlegendentry{\huge RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.021, 088.094) };
          % \addlegendentry{\huge SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.033, 072.607) };
          % \addlegendentry{\huge SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.077, 071.749) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.013, 061.524) };
          % \addlegendentry{\huge \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.009, 074.276) };
          \addlegendentry{\huge \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (000.012, 067.574) };
    \end{axis}
\end{tikzpicture}


==> figs/tiny/vit/fig.tex <==

\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.7cm,draw=none,font=\small, at={(-0.2,-0.2)}, xticklabel style={font=\tiny},
                 anchor=north west,
                 legend columns=3}]
          \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, ] coordinates { (000.000, 062.710) };
          \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt] coordinates { (000.040, 058.210) };
          \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, ] coordinates { (000.044, 058.190) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.055, 055.460) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.106, 065.820) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.041, 058.360) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.031, 057.910) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.030, 057.920) };
    \end{axis}
\end{tikzpicture}





\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.1,-0.2)}, xticklabel style={font=\tiny},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 065.280) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.044, 058.630) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.086, 058.350) };
          \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, ] coordinates { (000.092, 056.863) };
          \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, ] coordinates { (000.134, 066.400) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.045, 061.550) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.034, 060.810) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.034, 060.960) };
    \end{axis}
\end{tikzpicture}




\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=1cm,draw=none,font=\small, at={(-0.2,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 079.402) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.005, 052.635) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.013, 060.394) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.017, 053.087) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.062, 068.232) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, ] coordinates { (000.011, 058.650) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, ] coordinates { (000.013, 066.574) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.008, 061.757) };
    \end{axis}
\end{tikzpicture}



\begin{tikzpicture}[font=\sffamily, scale=0.5]
     \begin{axis}[grid, xlabel=Avg. Gap,
                 ylabel={$\mathcal{CS}_{GD}^{100}(\cdot, \mathcal{D}_f^{train})$},
                 legend style={column sep=0.5cm,draw=none,font=\small, at={(-0.0,-0.2)},
                 anchor=north west,
                 legend columns=3}]
          % \addlegendentry{\large Retraining}
          \addplot [blue, mark=star, mark size=4pt, forget plot] coordinates { (000.000, 087.784) };
          % \addlegendentry{\large FT}
          \addplot [RedViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.011, 051.872) };
          % \addlegendentry{\large RL}
          \addplot [BlueViolet, mark=*, mark size=4pt, forget plot] coordinates { (000.022, 064.515) };
          % \addlegendentry{\large SCRUB}
          \addplot [orange, mark=*, mark size=4pt, forget plot] coordinates { (000.026, 052.327) };
          % \addlegendentry{\large SALUN}
          \addplot [Brown, mark=*, mark size=4pt, forget plot] coordinates { (000.068, 076.719) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{GA}}
          \addplot [SeaGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.005, 049.997) };
          % \addlegendentry{\large \textbf{IEU} w/\texttt{Noisy}}
          \addplot [PineGreen, mark=*, mark size=4pt, forget plot] coordinates { (000.005, 052.536) };
          \addlegendentry{\large \textbf{IEU} w/\texttt{GA+Noisy}}
          \addplot [OliveGreen, mark=*, mark size=4pt, ] coordinates { (000.004, 053.512) };
    \end{axis}
\end{tikzpicture}


==> materials/tables/generation.tex <==
% \documentclass{standalone}
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{amsmath}
% \usepackage{moresize}
% \usepackage{multirow}
% \usepackage{makecell}



\begin{document}

\begin{tabular}{c|ccc}
    \hline \hline
           % & \multicolumn{2}{c}{ESD} & \multicolumn{2}{c}{SALUN} & \multicolumn{2}{c}{\textbf{IEU}} \\
           Method & FID ($\downarrow$) & Nudity score ($\downarrow$) & $\mathcal{RCD}_{Adam}$ ($\uparrow$) \\  \hline
           ESD & 0.880 & 0.413 & \textbf{538.022} \\
           ESD w/\texttt{GA} & 0.515 & 0.415 & {526.653} \\
           ESD w/\texttt{Noisy} & 0.510 & \textbf{0.224} & {524.057} \\
           ESD w/\texttt{GA+Noisy} & \textbf{0.428} & {0.330} & 517.166 \\\hline
           SALUN & 1.938 & 0.500 & \textbf{530.431} \\
           SALUN w/\texttt{GA} & 0.627 & 0.337 & {523.846} \\
           SALUN w/\texttt{Noisy} & 0.742 & 0.272 & {525.421} \\
           SALUN w/\texttt{GA+Noisy} & \textbf{0.350} & \textbf{0.250} & 506.544 \\
    \hline \hline
    
    \end{tabular}

\end{document}
